KETA: Kinematic-Phrases-Enhanced Text-to-Motion Generation via Fine-grained Alignment

Motion synthesis plays a vital role in various fields of artificial intelligence. Among the various conditions of motion generation, text can describe motion details elaborately and is easy to acquire, making text-to-motion(T2M) generation important. State-of-the-art T2M techniques mainly leverage diffusion models to generate motions with text prompts as guidance, tackling the many-to-many nature of T2M tasks. However, existing T2M approaches face challenges, given the gap between the natural language domain and the physical domain, making it difficult to generate motions fully consistent with the texts. We leverage kinematic phrases(KP), an intermediate representation that bridges these two modalities, to solve this. Our proposed method, KETA, decomposes the given text into several decomposed texts via a language model. It trains an aligner to align decomposed texts with the KP segments extracted from the generated motions. Thus, it's possible to restrict the behaviors for diffusion-based T2M models. During the training stage, we deploy the text-KP alignment loss as an auxiliary goal to supervise the models. During the inference stage, we refine our generated motions for multiple rounds in our decoder structure, where we compute the text-KP distance as the guidance signal in each new round. Experiments demonstrate that KETA achieves up to 1.19x, 2.34x better R precision and FID value on both backbones of the base model, motion diffusion model. Compared to a wide range of T2M generation models. KETA achieves either the best or the second-best performance.

==> hw.tex <==

% \begin{figure}[!tp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/hardware/lut_multiplier.pdf}
%     \vspace{-10pt}
%     \caption{The LUT-based multiplier. Each LUT multiplier is paired with a local table that prefetches and copies the intermediate results for multiplication, eliminating bank conflicts.}
%     \vspace{-15pt}
%     \label{fig:multiplier}
% \end{figure}

% \section{Buffered LUT-based Multiplication Architecture}

% \subsection{Overview of \hw}
% We present \hw, an end-to-end 3D-VGM accelerator featuring a buffered LUT-based Computing Engine that accelerates the computation of unimportant attention. \hw also includes additional architectural supports for the importance speculation in attention and the token-level similarity exploitation. Fig.~\ref{fig:hw-overview} shows our hardware overview.
% % \hw includes a Quantization Engine for quantization and the acquisition of the importance map, a Sparsification Engine for token reuse detection and output recovery, and a Computation Engine with FP16 PEs and LUT PEs to perform hybrid matrix multiplication.
% \subsection{The LUT-based Computing Engine}

% The LUT-based Computing Engine (LUT-based CE), as illustrated in Fig.~\ref{fig:hw-overview} (c), includes an FP16 Engine that manages FP-FP computations and a Mixed Engine that handles FP-INT multiplication with a LUT Buffer. The FP16 Engine deploys Element-Wise Units (EWU) to perform element-wise computations for quantization and sparsification. It also contains FP16 PEs that handle FP-FP matrix multiplication.

% The Mixed Engine contains an array of LUT PEs, as depicted in Fig.~\ref{fig:multiplier}. We employ the observation that the products between the 7-bit INT8 magnitudes and the 10-bit FP16 fractions can be precomputed, and they only occupy 128KB on-chip buffer size. By storing these precomputed products in the LUT Buffer, the FP-INT multiplication can be simplified into one lookup in LUT and one shift in the exponent, thus significantly reducing computations.

% However, bank conflicts must be solved since different LUT PEs may require the same intermediate results, which can stall our LUT-based CE and deteriorate efficiency. Our solution utilizes a group of local tables for each PE, whose multipliers share the same FP16 operands. Before each FP-INT MAC, we can prefetch the intermediate results by copying the table from the LUT Buffer to each PE's local tables. We leverage a double buffer for the local table so that the cost of our prefetch strategy can be hidden by the computation time of the multiplier.

% \subsection{Additional Architectural Support}

% Shown in Fig.~\ref{fig:hw-overview} (b), the Quantization Engine is mainly composed of a Prediction Unit (PU) and a Quantization Unit (QU). The PU aggregates input matrices via a Reduction Tree and multiplies the reduced matrices. It sorts the matrix, greedily selects the highest values with its Sort\&Select Unit(S\&SU), and stores the importance map in the Score Buffer. The QU quantizes $K$ and $V$ into the 8-bit one's complement representation, where the last 7 bits represent magnitude.

% Fig.~\ref{fig:hw-overview} (d) shows the Sparsification Engine, which is composed of a Sparsification Unit (SU), a Reorder \& Recover Unit (R\&RU), and an Index Buffer. After the query matrix $Q$ is generated, the SU exploits token-level similarity by computing the similarities and letting the Comparison Tree find the highest similarity, which is compared to the threshold in the T register. If the condition is satisfied, the Index Buffer will be updated. The R\&RU reorders $Q$ to sparsified $Q_c$ and recover $A$ from sparsified $A_c$. For both reordering and recovering, We traverse the index table, generating each index's source and destination addresses. Then, the data will be transferred according to the index and the addresses.




==> mapping.tex <==
% \section{Adaptive Grouping Strategy}
% \subsection{Algorithm-hardware Mapping Overview}

% We describe the MSA dataflow on \hw. Other phases in 3D-VGMs primarily involve FP-FP multiplication and element-wise operations and do not utilize specially devised engines.

% Initially, \(Q\) and \(K\) are reduced, and the importance map for \(P\) is generated in the Prediction Unit with the assistance of the Special Function Unit (SFU) and S\&SU. Concurrently, the SU and QU produce sparsified \(Q_c\) and quantized \(K_q\), respectively. The CE then computes $S$ and \(P\) row-by-row, leveraging both the FP16 Engine and Mixed Engine, guided by the importance map of \(P\). This row-by-row computation maximizes parallelism and enables the fusion of $P = Softmax\left(\frac{S}{\sqrt{d}}\right)
% $ and $A = PV$. As every \(t\) rows of \(S\) are computed in parallel, they are forwarded to the SFU to generate \(P\). This row slice of \(P\) is sent to the QE to obtain the importance map for \(A\). Here, we employ an adaptive grouping strategy for \(P\) (Sec.~\ref{sec:mapping:adaptive}). Subsequently, \(V\) columns are reordered and grouped based on the importance map for optimized resource utilization. Upon completing the full attention process, the Recovery Unit in the SE restores the \(A_c\) matrix to its original form.
% \subsection{Adaptive Grouping Strategy to Tame Workload Imbalance}

% \label{sec:mapping:adaptive}

% Randomly distributed similar tokens lead to workload imbalances in the sparsified \(Q_c\) matrix. For instance, during the attention computation phase, the workload of each PE is imbalanced, necessitating the compression of $Q_c$ to utilize computational resources fully. Such imbalance also occurs in the importance map speculation for \(A\), where we need to recover $P_c$ into $P$ for speculation fully, and 
% the distribution of $P_c$'s indices is random and uneven. Moreover, the recovery incurs significant memory overhead due to the separation of similar token pairs in different frames.

% We propose an adaptive grouping strategy to tame workload imbalance and integrate our frame-level and token-level speculations seamlessly. Instead of recovering \(P\) from \(P_c\), we directly reduce \(P_c\) for subsequent speculation, as our observations show that the value distribution in each column of \(A\) in even, allowing such strategy with no accuracy loss.

% % of the generated video since our overall strategy ensures nearly no accuracy loss. Also, such a strategy significantly accelerates the inference of 3D-VGMs, as detailed in Sec.~\ref{sec:eval:ablation}.

==> related.tex <==
\section{Related Work}


==> tables/algorithm-accuracy.tex <==
\begin{table}[]
\centering
\caption{Accuracy of \topic in 3D-VGMs.}
\vspace{-5pt}
\label{tab:accuracy}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{@{}c|c|c|c@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Component}} & \textbf{Method} & \textbf{CLIPSIM\ $\uparrow$} & \textbf{VBench\ $\uparrow$} \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Open-Sora-Plan v1.2}}} & Baseline & 0.196 & 0.305 \\ \cmidrule(l){2-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{\topic\ (Ours)}} & 0.196 & 0.305 \\  \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{CogVideoX-5B}}} & Baseline & 0.304 & 0.311 \\ \cmidrule(l){2-4}
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{\topic\ (Ours)}} & 0.307 & 0.312 \\
\bottomrule
\end{tabular}%
}
\vspace{-10pt}
\end{table}

==> tables/hardware-overhead.tex <==
\begin{table}[]
\centering
\caption{The area and power of \hw.}
\vspace{-5pt}
\label{tab:hardware-overhead}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}ccc|cc@{}}
\toprule
\multicolumn{3}{c|}{\textbf{Component}} & \textbf{Area ($mm^2$)} & \textbf{Power ($mW$)} \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{\textbf{Computing Engine}}} & \multicolumn{2}{c|}{16$\times$8 LUT PEs} & 1.23 & 47.10\\ \cmidrule(l){2-5}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{8$\times$8 FP16 PEs} & 2.71 & 323.07 \\ \cmidrule(l){2-5} 
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{4$\times$8 EWUs} & 0.04 & 3.58 \\ \midrule
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Quantization Engine}}} & \multicolumn{2}{c|}{Prediction Unit} & 0.02 & 1.40 \\ \cmidrule(l){2-5}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{Quantization Unit} & 0.03 & 1.89 \\  \midrule

\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{Spasification Engine}}} & \multicolumn{2}{c|}{Sparsification Unit} & 0.14 & 16.36 \\ \cmidrule(l){2-5}
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{Reorder and Recovery Unit} & 0.06 & 2.69 \\  
\midrule
\multicolumn{3}{c|}{\textbf{Special Function Unit}} & 0.23 & 11.02 \\ \midrule
\multicolumn{3}{c|}{\textbf{628KB On-chip buffer}} & 1.47 & 61.67 \\ \midrule
\multicolumn{3}{c|}{\textbf{Total (32$nm$)}} & 5.93 & 468.79 \\ \bottomrule
\end{tabular}%
}
\vspace{-10pt}
\end{table}
